Optimal individualized treatment regimes for survival data with competing risks

Precision medicine leverages patient heterogeneity to estimate individualized treatment regimens, formalized, data-driven approaches designed to match patients with optimal treatments. In the presence of competing events, where multiple causes of failure can occur and one cause precludes others, it is crucial to assess the risk of the specific outcome of interest, such as one type of failure over another. This helps clinicians tailor interventions based on the factors driving that particular cause, leading to more precise treatment strategies. Currently, no precision medicine methods simultaneously account for both survival and competing risk endpoints. To address this gap, we develop a nonparametric individualized treatment regime estimator. Our two-phase method accounts for both overall survival from all events as well as the cumulative incidence of a main event of interest. Additionally, we introduce a multi-utility value function that incorporates both outcomes. We develop random survival and random cumulative incidence forests to construct individual survival and cumulative incidence curves. Simulation studies demonstrated that our proposed method performs well, which we applied to a cohort of peripheral artery disease patients at high risk for limb loss and mortality.

==> Chapters/02_Proj1/01_chapters/3.Theory/lambda_star.tex <==
Equation \cref{eqn:AJhat_node} can be re-written in terms of distributions and hazard functions. We already know that $X_i = T_i \wedge C_i$ and $T_i = T_{1i} \wedge T_{2i}$. Let $H_i(t)$ be the CDF of $T_i$ and $G_i(t)$ be the CDF of $C_i$. 
%We also defined $N_i(s) = I(T_i \leq s, \epsilon_i = 1)$ where we assumed cause 1 is the priority cause, and $Y_i(s) = 1-N_i(s-)$ \citep{fine_proportional_1999}. \\ Then, $dN_i(s) = I(T_i = s, \epsilon_i = 1)$.
The counting process for cause-$j$ is given by $N_j(s) = \sum_{i=1}^{n} N_{ji}(s) = \sum_{i=1}^{n} 1(X_i \leq s, \, \delta_{ji} = 1)$, and the at-risk process is given by
$ K(s) = \sum_{i=1}^{n} K_i(s) = \sum_{i=1}^{n} 1(X_i \geq s)$. Then, taking the expectation of the risk set, we get the denominator to be
\begin{equation}
\begin{split}
\mathbb{E}(K_i(s)) &= \mathbb{E}(I(X_i \geq s)) = \Pr(X_i \geq s) = \Pr(T_i \wedge C_i \geq s) \\
&= \Pr(T_i \geq s, C_i \geq s) = \Pr(T_i \geq s) \Pr(C_i \geq s) \\
&=[1-\Pr(T_i < s)][1 - \Pr(C_i < s)]\\
&= [1-H_i(s)][1-G_i(s)],
\end{split}
\end{equation}
where we assume independence between overall failure and censoring times.
Next, we take the expectation of the counts of failures from cause $j$ at time $s$ to get the numerator:
\begin{equation}
    \begin{split}
\mathbb{E}(dN_{ji}(s)) &= \mathbb{E}(I(\delta_{ji} = 1, X_i = s)) \\ 
&= \mathbb{E}(I(\delta_{ji} = 1, T_i \wedge C_i = s, \epsilon_i = j)) \\ 
&= \Pr(\delta_{ji} = 1, T_i \wedge C_i = s, \epsilon_i = j, X_i \geq s) \\
&= \Pr(\delta_{ji} = 1, T_i \wedge C_i = s, \epsilon_i = j | X_i \geq s) \Pr(X_i > s)\\
&= \Pr(\delta_{ji} = 1, T_i \wedge C_i = s, \epsilon_i = j | T_i \geq s, C_i \geq s) \Pr(T_i > s, C_i > s)\\
&= \Pr(\delta_{ji} = 1, T_i \wedge C_i = s, \epsilon_i = j | T_i \geq s) [1-\Pr(T_i \leq s)][1 - \Pr(C_i \leq s)]\\
&= d\Lambda_{ji}(s)[1-H_i(s)][1-G_i(s)],
\end{split}
\end{equation}
where $d\Lambda_j(s)$ is the cause-$j$ specific hazard function defined in Equation \cref{eqn:dLambdaj}. The third equality holds because $X_i \geq s$ is a larger set than $X_i = s$, and the sixth equality holds because we assume independent censoring (i.e., being conditional on $T_i,C_i$ is the same as being conditional on just $T_i$ because $T_i \perp C_i$).



==> Chapters/02_Proj1/02_algorithms/CR_algorithms.tex <==
\newcommand{\algorithmOverview}{
\begin{algorithm}[H]
  \caption{The proposed ITR estimator accounting for competing risks.}
  \label{alg:Overview}
  \begin{algorithmic}
  \STATE \textbf{Input:} $Z_i, A_i, \tol$
  \STATE \textbf{Output:} $\dopt$
  \STATE %\ref{alg:RSF}
  \STATE For each individual $i$, given covariates $Z_i$ and small $0<\tol<1$, consider feasible treatments $a_i \in \psi(z_i) 
  \subset \mathcal{A}$ (we drop $i$ for simplicity):
  \begin{enumerate}
    \item Obtain $\survfunchat(\cdot|Z,A)$ via generalized random survival forest \citep{cho_multi-stage_2023}
    \item Obtain $\hat{F}_j(\cdot|Z,A)$ via random cumulative incidence forest (Algorithm \ref{alg:RCIF})
    \item Let optimal treatments for Phase 1 (overall survival) be $\valueonemaxTRUE = \argmax_{a \in \psi(z)}\valueone$
    \item Obtain overall survival treatment set $A^s = \{a \in \psi(Z): \valueone \ge (1- \tol)\valueonemaxTRUE\}$
        \begin{itemize}
            \item If $A^s$ is singleton, $A^s$ is the optimal treatment: $\dopt(Z) = A^s$.
            \item If $\#A^s > 1$, optimal treatment $\dopt(Z) = \argmin_{a \in \textit{A}^s} \valuetwo$.
        \end{itemize} 
    \end{enumerate}
  \STATE In other words, if $a_i \neq A^s_i$ for individual $i$, then individual $i$ stopped at either 
  \begin{itemize*}%[label={Phase \arabic*:}]
      \item \hspace{1em} Phase 1: $\valueone < (1-\tol)\valueonemaxTRUE$ or
      \item \hspace{1em} Phase 2: $\valueone \ge (1-\tol) \valueonemaxTRUE$ but $V_2(a = \dopt, Z) < V_2(a = a_i, Z)$
  \end{itemize*}\\
  and $A_i^s$ may have $\#A_i^s>1$.
\end{algorithmic}
\end{algorithm}
}

\newcommand{\algorithmRSF}{
\begin{algorithm}[H]
  \caption{RSF}
  \label{alg:RSF}
  \begin{algorithmic}
  \STATE \textbf{Input:} $Z_i, A_i$
  \STATE \textbf{Output:} $A_i^*$
  \STATE %\ref{alg:RSF}
  \STATE For each individual $i$, given covariates $Z_i$ and small $0<\tol<1$, consider feasible treatments $a_i \in \psi(z_i) \subset \mathcal{A}$:
  \STATE
  \STATE hi
  \STATE
\end{algorithmic}
\end{algorithm}
}

\newcommand{\algorithmgRCIF}{%

\begin{algorithm}[H]
  \caption{the random cumulative incidence forest estimator}
  \label{alg:RCIF}
  \begin{algorithmic}
  \STATE Result: random cause-j cumulative incidence forest $\hat{F}_j(\cdot|Z,A)$
  \STATE Parameters: the number of trees $n_{\text{tree}}$, the number of minimum terminal node size $n_{\text{min}}$
  \STATE \textbf{Input:} $\{(X_i, \delta_{ji}, Z_i, A_i)\}_{i=1}^n$
  \STATE \textbf{Output:} $\hat{F}_j(\cdot|Z,A=a)$
  \STATE 
  \STATE for \underline{treatment arm} $a \in \mathcal{A}$ \textbf{do} \\
  \STATE \quad for \underline{tree $w = 1, 2, \ldots, n_{\text{tree}}$} \textbf{do} \\
  \STATE \quad \quad Partition the feature space with the input data $\{(I(t\leq X_i), \delta_{ji}, Z_i)\}_{i:a_i=a}$ via Gray's test \cref{grays_test} or MD \citep{cho_multi-stage_2023} until node size $< 2n_{\text{min}}$ \\
  \STATE \quad \quad Obtain the terminal node cumulative incidence probability $\hat{F}^a_{j,\{w\}}(t | Z)$ via Aalen-Johanson estimator \cref{AJ_estimator} \\
  \STATE \quad Obtain the random cumulative incidence forest estimator \\
  \STATE \quad $\hat{F}_j(\cdot | Z, A = a) = \frac{1}{n_{\text{tree}}} \sum_{w=1}^{n_\text{tree}} \hat{F}_{j,\{w\}}^{a}(t | Z)$ \\

\end{algorithmic}
\end{algorithm}
}

==> Chapters/02_Proj1/02_theorems/02_assumptions/Assumptions.tex <==
% Assumptions
\newcommand{\RFassump}{
\input{Chapters/02_Proj1/02_theorems/02_assumptions/CR_assumptions}
% Assumptions for Forest Consistency
Below are assumptions used for consistency of both forests. Assumptions \ref{assump:Cho1}-\ref{assump:Cho3} are necessary and realistic for the tree-based estimator terminal node size and splitting rules. Assumption \ref{assump:Cho1} requires the terminal node size to be not only sufficiently large absolutely but also sufficiently small relative to the sample size. Assumption \ref{assump:Cho2} follows from Definition \ref{def:regsplotalphatree}. Assumption \ref{assump:Cho3} adds smoothness to the survival function and censoring cumulative distribution function. Assumption \ref{assump:CuiAssump2} follows from \cite{cui_tree_2017} and \cite{wager_adaptive_2016}, which allows for dependency between covariates. Thus, non-hyper-rectangular or categorical history spaces are allowed with this assumption. Assumption \ref{khbddtv} is necessary for the random cumulative incidence forest because there is non-differentiability of the treatment policy.
\assumpsForestconsistency
}

\newcommand{\ITRassump}{
\input{Chapters/02_Proj1/02_theorems/02_assumptions/CR_assumptions}
% Assumptions for ITR Consistency
Below are assumptions for the proposed estimator for consistency. We assume bounding in Assumptions \ref{assump:boundeddensity}-\ref{assump:boundedV0} to account for nonregularity of the value function. This is a necessary and standard assumption for non-regularity conditions.
\assumptionsITRconsistency
}

==> Chapters/02_Proj1/02_theorems/02_assumptions/CR_assumptions.tex <==
% assumptions for RCIF Adaptive Bounds!
\newcommand{\ASSUMPrcifconsisBoundedTau}{
\begin{assumption}
\label{assump:CuiAssump1}
There exists a fixed maximum follow-up time $0 < \tau < \infty$ and a constant $\tauUB \in (0, 1)$, such that $Pr(X_\tau \geq \tau | Z = z) \geq \tauUB$, for all $z \in \mathcal{Z}$.
\end{assumption}
}

\newcommand{\ASSUMPrcifconsisBoundedCovDistrO}{
\begin{assumption}
    \label{assump:CuiAssump2}
    The covariates $Z \in [0; 1]^d$ are distributed according to a density function $p(\cdot)$ satisfying $1/\assumpcovbound \leq p(z) \leq \assumpcovbound$, for all $z$ and some $\assumpcovbound \geq 1$.
\end{assumption}
}

\newcommand{\ASSUMPrcifconsisBoundedBelowKO}{
\begin{assumption}
\label{assump:CuiAssump3}
Assume that the minimum terminal node size $k$ is bounded below such that
\[
\lim_{n \to \infty} \frac{\log(n) \max\{\log(d), \log \log(n)\}}{k} = 0.
\]
\end{assumption}
}

\newcommand{\ASSUMPrcifconsisLipschitzCtsO}{
\begin{assumption}
\label{assump:CuiAssump4}
For any fixed time point $t$, the distribution function for failure from any cause $H(t | z)$ is $L_1$-Lipschitz continuous in terms of $z$, and the cause-$j$ specific hazard function $\lambda_j(t | z)$ is $L_2$-Lipschitz continuous in terms of $z$;
that is, 
\begin{equation*}
|H(t | z_1) - H(t | z_2)| \leq L_1 \norm{z_1 - z_2}
\text{ and }
|\lambda_j(t | z_1) - \lambda_j(t | z_2)| \leq L_2 \norm{z_1 - z_2}, 
\end{equation*}
where $|| \cdot ||$ is the Euclidean norm.
\end{assumption}
}

\newcommand{\ASSUMPrcifconsisHazardBoundO}{
\begin{assumption}
\label{assump:HazardBound}
Assume $\lambda_j(s|z)$ is bounded from $0$ to $\tau$ by some constant  $\assumphazbound$. Then, $\max_{s} \lambda_j(s|z) \leq \assumphazbound.$
\end{assumption}
}

\newcommand{\assumptionsRCIFadaptiveboundsO}{
%\ASSUMPrcifconsisBoundedTau
%\ASSUMPrcifconsisBoundedCovDistr
\ASSUMPrcifconsisBoundedBelowK
\ASSUMPrcifconsisLipschitzCts
\ASSUMPrcifconsisHazardBound
}

\newcommand{\assumpsForestconsistencyO}{
\input{Chapters/02_Proj1/02_theorems/02_assumptions/Cho_assumptions1_5}
}

% assumptions for ITR consistency
\newcommand{\assumptionsITRconsistencyO}{
\begin{assumption}
\label{assump:boundeddensity}
Define the random function $B(a,Z) = \valueoneTRUE - (1-\tol)\valueonemaxTRUE$, $a \in \mathcal{A}$. Assume $B(a,Z)$ has continuous, bounded densities at 0, for each $a \in \mathcal{A}$.
\end{assumption}

\begin{assumption}
\label{assump:boundedV0}
    $\sup_{a,Z} \left\| \valueTRUE \right\|$ is bounded by some $\sevenbound < \infty$.
\end{assumption}
}


==> Chapters/02_Proj1/02_theorems/02_assumptions/Cho_assumptions1_5.tex <==
\begin{assumption}[Terminal node size, polynomial]
\label{assump:Cho1}
The minimum size \( n_{\text{min}} \) of the terminal nodes grows at the rate \( n_{\text{min}} \bowtie n^\beta \), \( \frac{1}{2} < \beta < 1 \), where \( a \bowtie b \) implies that both \( a = O(b) \) and \( b = O(a) \).
\end{assumption}

\begin{assumption}
[\( \alpha \)-regular and random-split trees]
\label{assump:Cho2}
Trees are \( \alpha \)-regular and random-split with a constant \( 0 < \psi < 1 \).
\end{assumption}

\begin{assumption}[Lipschitz continuous and bounded survival and censoring cumulative densities]
\label{assump:Cho3}
There exist constants \( \lipS \) and \( \lipG \) such that \( |\survfunc(t | h_1) - \survfunc(t | h_2)| \leq \lipS\|h_1 - h_2\| \) and \( |G(t | h_1) - G(t | h_2)| \leq \lipG \|h_1 - h_2\| \) for all \( h_1, h_2 \in \history \), \( t \in [0, \tau] \), where \( G \) is the censoring cumulative distribution function (CDF) and \( \survfunc(\tau^- \mid \histlower)G(\tau^- \mid \histlower) > c_1 \) for all \( \histlower \) and some constant \( c_1 > 0 \).
\end{assumption}

%\input{Chapters/02_Proj1/02_theorems/02_assumptions/CR_assumptions}
%\ASSUMPrcifconsisBoundedCovDistr
\begin{assumption}
    \label{assump:CuiAssump2}
    The covariates $Z \in [0; 1]^d$ are distributed according to a density function $p(\cdot)$ satisfying $1/\assumpcovbound \leq p(z) \leq \assumpcovbound$, for all $z$ and some $\assumpcovbound \geq 1$.
\end{assumption}

\begin{assumption}
\label{khbddtv}
The kernel \( \kernel \) for the random cumulative incidence forest has bounded total variation. Specifically, there exists a constant \( C \) such that the total variation of \( \kernel \) satisfies
\[
\int_{-\infty}^{\infty} \abs{\kernel^\prime(x)} \, dx \leq C,
\]
where \( \kernel^\prime(x) \) denotes the derivative of the kernel \( \kernel \).
\end{assumption}

==> Chapters/02_Proj1/02_theorems/Forest/Consistency/Lemmas/PropProofs/Prop5Proof.tex <==
\begin{comment}
\begin{proof}[Proof of Proposition \ref{prop:ChoProp6}]

The Vapnik-Chervonenkis (VC)-dimension of any axis-aligned rectangles in $\mathbb{R}^d$ can be shown to be $2d$. By Theorem 9.2 of Kosorok (2007), for any VC-class of sets $C$, the collection $\mathbb{1}(C)$ of all the corresponding indicator functions has a bounded covering number $N(\epsilon, \mathbb{1}(C), L_r(P)) \leq K_1 V(C)(4e)V(C)^\epsilon - r(V(C)-1)$, where $V(\cdot)$ denotes the VC-dimension, and $K_1 < 1$ is some universal constant. Thus, the collection $\mathbb{1}(C_{\text{TREE}})$ of the unnormalized tree kernels has a bounded covering number: $N(\epsilon, \mathbb{1}(C_{\text{TREE}}), L_2(P)) \leq K_2 \epsilon^{-(4d-2)}$, for some constant 
$K_2 < 1$. This immediately implies that the class of tree kernels have bounded entropy integrals

$$
\left(\int_{0}^{1} N(\epsilon, \mathbb{1}(C_{\text{TREE}}),L_2(P)) d\epsilon = 1\right)
$$

and thus is Donsker.

Next, since a forest kernel is simply a convex hull of the tree kernels, i.e., $\text{conv}(\mathbb{1}(C_{\text{TREE}})) = \left\{ \sum_{i=1}^{m} \alpha_i 1(c_i) : \sum_{i=1}^{m} \alpha_i = 1, \alpha_i \geq 0, c_i \in C_{\text{TREE}}, i = 1, 2, \ldots, m \right\}$, by Theorem 9.4 of Kosorok (2007), $N_{f}(\epsilon, \text{conv}(\mathbb{1}(C_{\text{TREE}})),L_2(P)) \leq K_3 \epsilon^{-(2 - \frac{1}{d})}$ for some constant $K_3 < 1$. This implies that the unnormalized forest kernels are also Donsker. 
\end{proof}
\end{comment}


==> Chapters/02_Proj1/02_theorems/Forest/Forest_Details.tex <==
We now provide adaptive concentration bounds for the random cumulative incidence forests. Note that the following shows consistency over time $t$ only, not over $\histlower \in \history$.
Let $\scriptNode = \{ \Nodeu \}_{u \in U}$ be the set of terminal nodes obtained by fitting a single tree, where $U$ is a set of indices, $Z = \bigcup_{u \in U} \Nodeu$, and $\Nodeu \cap \Node_l = \emptyset$ for any $u \neq l$. Recursive partitioning is a critical component of tree-based survival models, where a $d$-dimensional feature space $Z$ is partitioned into terminal nodes. In other words, $\scriptNode$ is a partition of $Z$. Following the traditional tree-building process in \cite{breiman1984classification}, binary splitting rules are used, and all terminal nodes $\Nodeu$ are non-overlapping hyper-rectangles \citep{wager_adaptive_2016, cui_consistency_2022, cho_multi-stage_2023}. A set of $B$ trees are fitted in a traditional survival forest model \citep{ishwaran_random_2008}. 
Hence, our tree model yields $\{ \Nodeu, \hat{\cuminc}_{\Nodeu,n}\}_{u \in U}$, and our forest constructs a collection of partitions $\{\{ \Nodeu^b, \hat{\cuminc}_{\Nodeu,n} \}_{u \in U_b}\}^B_{b=1}$.

The AJ estimator for any node $\Nodeu$ is
\begin{equation}
\label{eqn:AJhat_node}
\hat{\cuminc}_{\Nodeu,n}(t) = 
\sum_{s \leq t}
\frac{
\survfunchatNodeu(s-)
    \sum_{i=1}^n I{\{ \delta_{1i} = 1, X_i = s  \}}
    I{\{ Z_i \in \Nodeu \}}}{\sum_{i=1}^n I{\{ X_i \geq s \}} I{\{ Z_i \in \Nodeu \}}},
\end{equation} where the Kaplan-Meier estimator for overall survival in node $\Nodeu$ at time $t$ is given by 
$\survfunchatNodeu(t)$.
We know that the Kaplan-Meier estimator in the survival forest is consistent. To quantify within-node estimation performance, let $\cuminc_\Node(t) = \frac{1}{\mu(\Node)} \int_{z\in \Node} \cuminc(t | z) dP(z)$ be the averaged CIF within any node $\Node$, where $\cuminc(t|z)$ is defined in Equation \cref{eqn:CIF_def}, $P$ is the distribution of $Z$, and $\mu(\Node) = \int_{z\in \Node} dP(z)$ is the measure of node $\mathcal{Z}$.

\input{Chapters/02_Proj1/01_chapters/3.Theory/lambda_star}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> layout.tex <==
% Use proper margins.
\geometry{letterpaper,left=1in,top=1in,right=1in,bottom=1in,nohead}

% double-space text
\doublespacing

%\MakeUppercase{\chaptertitlename} \thechapter

% Center chapter titles, omit page numbers.
\titleformat{\chapter}[display]{\fillast\bfseries}{}{-11pt}{\singlespacing}

% Section titles
\titleformat{\section}{\normalfont\fontsize{12}{15}\bfseries}{\thesection}{1em}{}
\titleformat{\subsection}{\normalfont\fontsize{12}{15}\bfseries}{\thesubsection}{1em}{}

% Extend to 2in top margins
% Leave 22pts = 2x font size after heading
\titlespacing{\chapter}{0in}{0.62in}{22pt}

% Indent paragraphs four spaces throughout the thesis/dissertation.
\setlength{\parindent}{4ex}

% Tweak spacing of paragraph labels.
\titlespacing{\paragraph}{0in}{0.08in}{0.07in}

% We want numbered subsubsections
\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}

% We need to double-space between footnotes.
\setlength{\footnotesep}{13pt}

% We don't want crazy vertical spacing.
\raggedbottom

% We don't want abandoned words.
\clubpenalty=10000 
\widowpenalty=10000

% Prevent awkward hyphenations.
\hyphenation{Raj-kumar}


==> macros.tex <==
% DJL: commented out the following... we don't want cite replaced with citep
% default: cite with (Name, year)
%\renewcommand{\cite}{\citep}

\usepackage{longtable}
%%
%% some convenient packages
%%
\usepackage{physics}  %% (p)dv for (partial) derivatives
\usepackage{booktabs}
\usepackage[section]{placeins}
%\usepackage{morefloats} % SAR (2020) commented out
\usepackage{float} % SAR (2020) added
\usepackage{subfig} % SAR (2020) added
\usepackage{amssymb}
\usepackage{setspace}
\usepackage{rotating}
\usepackage{graphicx}
\usepackage{booktabs} 
\usepackage{stmaryrd}
\usepackage{times}
\usepackage{bm}
\usepackage{indentfirst}
\usepackage{natbib}
\usepackage{amsmath}
\usepackage{enumerate}
\usepackage{enumitem}
\usepackage{array}
\usepackage{multicol}

\allowdisplaybreaks   %% allows align environment to break page

% common abbreviations
\newcommand{\eg}{{\it e.g.}\xspace}
\newcommand{\ie}{{\it i.e.}\xspace}
\newcommand{\etc}{{\it etc.}\xspace}
\newcommand{\etal}{\emph{et~al}\mbox{.}\xspace}
\newcommand{\vs}{{vs\mbox{.}}\xspace}

% common Math notation
\newcommand{\NAT}[0]{\mathbb{N}\xspace}
\newcommand{\fun}[1]{\mathit{#1}} % typeset as function name
\newcommand{\setsize}[1]{\left| #1 \right|}
\newcommand{\setdef}[2]{\left\{ #1 \ \left|\  #2\right.\right\}}
\newcommand{\dispsum}[0]{\displaystyle\sum}

\newcommand{\defeq}[0]{\triangleq}
\renewcommand{\mod}{\operatorname{mod}}

%% Macros for literature review
\newcommand*{\Gam}{\mathop{\mathrm{Gamma}}\nolimits}
\newcommand*{\Exp}{\mathop{\mathrm{Exponential}}\nolimits}
\newcommand*{\Ber}{\mathop{\mathrm{Bernoulli}}\nolimits}

% cross referencing equations 
\usepackage{cleveref} % For intelligent cross-referencing
% Define the format for equation references
\crefformat{equation}{(#2#1#3)}

%% Macros for paper 1
\newcommand*{\diag}{\mathop{\mathrm{diag}}\nolimits}
\newcommand*{\bernoulli}{\mathop{\mathrm{Bernoulli}}\nolimits}
\newcommand*{\N}{\mathop{\mathrm{N}}\nolimits}
\newcommand*{\G}{\mathop{\mathrm{Gamma}}\nolimits}
\newcommand*{\W}{\mathop{\mathrm{W}}\nolimits}
\newcommand*{\IW}{\mathop{\mathrm{IW}}\nolimits}
\newcommand*{\TN}{\mathop{\mathrm{TN}}\nolimits}
\newcommand*{\E}{\mathop{\mathrm{E}}\nolimits}
\newcommand*{\Var}{\mathop{\mathrm{Var}}\nolimits}
\newcommand*{\Cov}{\mathop{\mathrm{Cov}}\nolimits}
\newcommand*{\Cor}{\mathop{\mathrm{Cor}}\nolimits}
\newcommand*{\Corr}{\mathop{\mathrm{Corr}}\nolimits}
\newcommand*{\blkdiag}{\mathop{\mathrm{blkdiag}}\nolimits}
\newcommand*{\vect}{\mathop{\mathrm{vec}}\nolimits}
\newcommand*{\POS}{\mathop{\mathrm{POS}}\nolimits}

%% Macros for paper 2
\newcommand*{\CI}{\pi_{\text{CI}}}
\newcommand*{\APP}{\pi_{\text{APP}}}
\newcommand*{\LKJ}{\pi_{\text{LKJ}}}
\newcommand*{\HC}{\pi_{\text{HC}}}
\newcommand*{\CIHC}{\pi_{\text{CIHC}}}
\newcommand*{\pos}{\text{POS}}

%% Macros for paper 3
\def\R{{\mathbb{R}}}
\DeclareMathOperator{\logit}{logit}
\DeclareMathOperator{\expit}{expit}
\DeclareMathOperator{\DY}{\pi_{\text{DY}}}
\DeclareMathOperator{\HPP}{\pi_{\text{HPP}}}
\newcommand{\appropto}{\mathrel{\vcenter{
  \offinterlineskip\halign{\hfil$##$\cr
    \propto\cr\noalign{\kern2pt}\sim\cr\noalign{\kern-2pt}}}}}






% references
\newcommand{\chref}[1]{Chapter~\ref{ch:#1}\xspace}
\newcommand{\chrefs}[2]{Chapters~\ref{ch:#1} and~\ref{ch:#2}\xspace}
\newcommand{\secref}[1]{Section~\ref{sec:#1}\xspace}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}\xspace}
\newcommand{\figrefi}[2]{Figure~\ref{fig:#1}(#2)\xspace}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}\xspace}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}\xspace}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}\xspace}
\newcommand{\defref}[1]{Definition~\ref{def:#1}\xspace}
\newcommand{\exref}[1]{Example~\ref{ex:#1}\xspace}
\newcommand{\equref}[1]{Equation~(\ref{eq:#1})\xspace}
\newcommand{\inequref}[1]{Inequality~(\ref{eq:#1})\xspace}
\newcommand{\lstref}[1]{Listing~\ref{lst:#1}\xspace}
\newcommand{\pref}[1]{page~\pageref{p:#1}\xspace}
% citations


% special footnotes

% from http://help-csli.stanford.edu/tex/latex-footnotes.shtml
\long\def\symbolfootnote[#1]#2{\begingroup%
\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}

% Theorems, etc.

\newtheoremstyle{mylemthm}% hnamei 
        {6pt}% hSpace abovei 
        {3pt}% hSpace belowi 
        {\slshape}% hBody fonti 
        {}% hIndent amounti1
        {\bfseries}% hTheorem head fonti 
        {.}% hPunctuation after theorem headi 
        {.5em}% hSpace after theorem headi2
        {}% hTheorem head spec (can be left empty, meaning `normal')i

\theoremstyle{mylemthm}
\newtheorem{assumption}{Assumption}[chapter]
\newtheorem{condition}{Condition}[chapter]

%\theoremstyle{definition}

%% "inherent" from xxexample, but place box at the end of example.
\newenvironment{example}{
\begin{xxexample}
}{
\rightparend{$\Diamond$}
\end{xxexample}
}
% \qed   \sqbullet \blackdiamond \vartriangleleft


% DJL: I added more macros below 

% I think just these ones should suffice
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

% you'll have to check that everything is numbered correctly
\newtheorem{theorem}{Theorem}[chapter]
\newtheorem{lemma}{Lemma}[chapter]
\newtheorem{prop}{Proposition}[chapter]
\newtheorem{corollary}{Corollary}[chapter]
\newtheorem{remark}{Remark}[chapter]
\newtheorem{definition}{Definition}[chapter]

% here's one more
\newcommand{\T}{\intercal}

% and one more
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}

% last one for real
\newcommand{\pn}{\mathbb{E}_n}

% and one more
\newcommand{\rp}{\mathbb{R}^p}

% added by MTL (2019)
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator{\imp}{imp}
\DeclareMathOperator{\opt}{opt}
\DeclareMathOperator{\sign}{sign}
\newcommand{\bignorm}[1]{\left\lVert#1\right\rVert}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\meani}{\displaystyle{\frac{1}{n}\sum_{i=1}^{n}}}
\newcommand{\sumi}{\displaystyle{\sum_{i=1}^{n}}}
\newcommand{\bhat}{\hat{\beta}}
\newcommand{\btil}{\tilde{\beta}}
\newcommand{\Dhat}{\hat{\Delta}}
\newcommand{\Szsig}{S^{0}_{\sigma}}

%% Added by SAR (2020):

% for wide hat
\usepackage{scalerel,stackengine}
\stackMath
\newcommand\reallywidehat[1]{%
\savestack{\tmpbox}{\stretchto{%
  \scaleto{%
    \scalerel*[\widthof{\ensuremath{#1}}]{\kern.1pt\mathchar"0362\kern.1pt}%
    {\rule{0ex}{\textheight}}%WIDTH-LIMITED CIRCUMFLEX
  }{\textheight}% 
}{2.4ex}}%
\stackon[-6.9pt]{#1}{\tmpbox}%
}

% for commenting
\newcommand{\sarah}[1]{\textcolor{green}{(Sarah: #1)}}

% to name rows of subfigs
% https://tex.stackexchange.com/questions/239715/add-titles-for-rows-and-columns-in-a-subfloat/239809
\usepackage{mwe}
\newlength{\tempheight}
\newlength{\tempwidth}
\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\tempheight][c]{\textbf{#1}}}}
\newcommand{\columnname}[1]% #1 = text
{\makebox[\tempwidth][c]{\textbf{#1}}}

% Begin code from  PDF -> Latex (Rmd generated tex file)
\usepackage{color}
\usepackage{fancyvrb}
\newcommand{\VerbBar}{|}
\newcommand{\VERB}{\Verb[commandchars=\\\{\}]}
\DefineVerbatimEnvironment{Highlighting}{Verbatim}{commandchars=\\\{\}}
% Add ',fontsize=\small' for more characters per line
\usepackage{framed}
\definecolor{shadecolor}{RGB}{248,248,248}
\newenvironment{Shaded}{\begin{snugshade}}{\end{snugshade}}
\newcommand{\KeywordTok}[1]{\textcolor[rgb]{0.13,0.29,0.53}{\textbf{#1}}}
\newcommand{\DataTypeTok}[1]{\textcolor[rgb]{0.13,0.29,0.53}{#1}}
\newcommand{\DecValTok}[1]{\textcolor[rgb]{0.00,0.00,0.81}{#1}}
\newcommand{\BaseNTok}[1]{\textcolor[rgb]{0.00,0.00,0.81}{#1}}
\newcommand{\FloatTok}[1]{\textcolor[rgb]{0.00,0.00,0.81}{#1}}
\newcommand{\ConstantTok}[1]{\textcolor[rgb]{0.00,0.00,0.00}{#1}}
\newcommand{\CharTok}[1]{\textcolor[rgb]{0.31,0.60,0.02}{#1}}
\newcommand{\SpecialCharTok}[1]{\textcolor[rgb]{0.00,0.00,0.00}{#1}}
\newcommand{\StringTok}[1]{\textcolor[rgb]{0.31,0.60,0.02}{#1}}
\newcommand{\VerbatimStringTok}[1]{\textcolor[rgb]{0.31,0.60,0.02}{#1}}
\newcommand{\SpecialStringTok}[1]{\textcolor[rgb]{0.31,0.60,0.02}{#1}}
\newcommand{\ImportTok}[1]{#1}
\newcommand{\CommentTok}[1]{\textcolor[rgb]{0.56,0.35,0.01}{\textit{#1}}}
\newcommand{\DocumentationTok}[1]{\textcolor[rgb]{0.56,0.35,0.01}{\textbf{\textit{#1}}}}
\newcommand{\AnnotationTok}[1]{\textcolor[rgb]{0.56,0.35,0.01}{\textbf{\textit{#1}}}}
\newcommand{\CommentVarTok}[1]{\textcolor[rgb]{0.56,0.35,0.01}{\textbf{\textit{#1}}}}
\newcommand{\OtherTok}[1]{\textcolor[rgb]{0.56,0.35,0.01}{#1}}
\newcommand{\FunctionTok}[1]{\textcolor[rgb]{0.00,0.00,0.00}{#1}}
\newcommand{\VariableTok}[1]{\textcolor[rgb]{0.00,0.00,0.00}{#1}}
\newcommand{\ControlFlowTok}[1]{\textcolor[rgb]{0.13,0.29,0.53}{\textbf{#1}}}
\newcommand{\OperatorTok}[1]{\textcolor[rgb]{0.81,0.36,0.00}{\textbf{#1}}}
\newcommand{\BuiltInTok}[1]{#1}
\newcommand{\ExtensionTok}[1]{#1}
\newcommand{\PreprocessorTok}[1]{\textcolor[rgb]{0.56,0.35,0.01}{\textit{#1}}}
\newcommand{\AttributeTok}[1]{\textcolor[rgb]{0.77,0.63,0.00}{#1}}
\newcommand{\RegionMarkerTok}[1]{#1}
\newcommand{\InformationTok}[1]{\textcolor[rgb]{0.56,0.35,0.01}{\textbf{\textit{#1}}}}
\newcommand{\WarningTok}[1]{\textcolor[rgb]{0.56,0.35,0.01}{\textbf{\textit{#1}}}}
\newcommand{\AlertTok}[1]{\textcolor[rgb]{0.94,0.16,0.16}{#1}}
\newcommand{\ErrorTok}[1]{\textcolor[rgb]{0.64,0.00,0.00}{\textbf{#1}}}
\newcommand{\NormalTok}[1]{#1}
% End code from  PDF -> Latex (Rmd generated tex file)

% Personal project commands
\input{0.header_thesis}
